Regularization Matters: Generalization and Optimization of Neural Nets v.s. their Induced Kernel

Recent works have shown that on sufficiently over-parametrized neural nets, gradient descent with relatively large initialization optimizes a prediction function in the RKHS of the Neural Tangent Kernel (NTK). This analysis leads to global convergence results but does not work when there is a standard $\ell_2$ regularizer, which is useful to have in practice. We show that sample efficiency can indeed depend on the presence of the regularizer: we construct a simple distribution in d dimensions which the optimal regularized neural net learns with $O(d)$ samples but the NTK requires $\Omega(d^2)$ samples to learn. To prove this, we establish two analysis tools: i) for multi-layer feedforward ReLU nets, we show that the global minimizer of a weakly-regularized cross-entropy loss is the max normalized margin solution among all neural nets, which generalizes well; ii) we develop a new technique for proving lower bounds for kernel methods, which relies on showing that the kernel cannot focus on informative features. Motivated by our generalization results, we study whether the regularized global optimum is attainable. We prove that for infinite-width two-layer nets, noisy gradient descent optimizes the regularized neural net loss to a global minimum in polynomial iterations.

==> comparison.tex <==
\begin{wrapfigure}{R}{0.20\textwidth}
	\includegraphics[width=0.19\textwidth]{figures/dist_plot.png}
	\caption{60 sampled points from $\cD$ in 3 dimensions. Red points denote negative examples and blue points denote positive examples.}
	\label{fig:cDvis}
\end{wrapfigure}
\label{subsec:classificationcompare}
Importantly, the $\ell_1$-max margin on the lifted feature space is obtainable by optimizing a finite neural network. We compare this to the $\ell_2$ margin attainable via kernel methods. Following the setup of~\eqref{eq:l1svm}, we define the kernel problem over $\alpha \in \spacetwo(\sph)$:
\begin{align}
\begin{split}
\opt_{\ell_2}\triangleq& \max_{\alpha} \min_{i\in [n]} y_i\langle \alpha, \varphi(x_i)\rangle\\
& \subj  \sqrt{\kappa}\|\alpha\|_2 \le 1\label{eq:kernel}
\end{split}
\end{align}
where $\kappa \triangleq \vol(\sph)$. (We scale $\|\alpha\|_2$ by $\sqrt{\kappa}$ to make the lemma statement below cleaner.) First, $\gamma_{\ell_2}$ can be used to obtain a standard upper bound on the generalization error of the kernel SVM. Following the notation of Section~\ref{sec:generalizationdeep}, we will let $L_{\ell_2\textup{-svm}}$ denote the 0-1 population classification error for the optimizer of~\eqref{eq:kernel}.
\begin{lemma}\label{lem:generror-l2-svm}
	In the setting of Proposition~\ref{prop:genbound}, with probability at least $1-\delta$, the generalization error of the kernel SVM with \relu~feature (defined in~\eqref{eq:kernel}) satisfies
	\begin{align}
	L_{\ell_2\textup{-svm}} \lesssim \frac{C}{\gamma_{\ell_2}\sqrt{dn}} + \epsilon_{\ell_2}
	\label{eq:generror-l2-svm}
	\end{align}
	where $\epsilon_{\ell_2} \triangleq \sqrt{\frac{\log \max\left \{\log_2 \frac{C}{\sqrt{d}\gamma_{\ell_2}}, 2\right\}}{n}} + \sqrt{\frac{\log (1/\delta)}{n}}$ is typically a lower-order term.
\end{lemma}
The bound above follows from standard techniques~\citep{bartlett2002rademacher}, and we provide a full proof in Section~\ref{subsec:kernelgenbound}. We construct a data distribution for which this lemma does not give a good bound for kernel methods, but Corollary~\ref{cor:margingeneralization} does imply good generalization for two-layer networks. 
\begin{theorem}
	\label{thm:l1-l2}
	There exists a data distribution $\pdata$ such that the $\ell_1$ SVM with~\relu~features has a good margin: 
$
	\gamma_{\ell_1} \gtrsim 1
$
	and with probability $1- \delta$ over the choice of i.i.d. samples from $\pdata$, obtains generalization error 
	\begin{align*}
	L_{\ell_1\textup{-svm}} \lesssim \sqrt{\frac{d \log n }{n}} + \epsilon_{\ell_1}
	\end{align*}
	where $\epsilon_{\ell_1} \triangleq  \sqrt{\frac{\log (1/\delta)}{n}}$ is typically a  lower order term. Meanwhile, with high probability the $\ell_2$ SVM has a small margin: 
$
	\gamma_{\ell_2} \lesssim \max\left\{\sqrt{\frac{\log n}{n}}, 1/d\right\}
$
	and therefore the generalization upper bound from Lemma~\ref{lem:generror-l2-svm} is at least
	\begin{align*}
	\Omega\left(\min\left \{1,  d \sqrt{\frac{\log n}{n}}\right \} \right)
	\end{align*}
	In particular, the $\ell_2$ bound is larger than the $\ell_1$ bound by a $\Omega(\sqrt{d})$ factor.
\end{theorem}

Although Theorem~\ref{thm:l1-l2} compares upper bounds, our construction highlights properties of distributions which result in better neural network generalization than kernel method generalization. Furthermore, in Section~\ref{sec:experiments} we empirically validate the gap in generalization between the two methods.

We briefly overview the construction of $\pdata$ here. The full proof is in Section~\ref{subsec:class-compare-proofs}. 

\paragraph{Proof sketch for Theorem~\ref{thm:l1-l2}.}
We base $\pdata$ on the distribution $\cD$ of examples $(x,y)$ described below. Here $e_i$ is the i-th standard basis vector and we use $x^\top e_i$ to represent the $i$-coordinate of $x$ (since the subscript is reserved to index training examples). First, for any $\forall k \ge 3, x^\top e_k \sim \cN(0,1)$ and for $x^\top e_1, x^\top e_2$ and $y$, choose
\\\\\\\begin{align*}
\begin{array}{llll}
y = +1,  & x^\top e_1 = +1, & x^\top e_2 = +1 & \textup{ w/ prob. } 1/4 \\
y = +1, & x^\top e_1 = -1, &x^\top e_2 = -1 & \textup{ w/ prob. } 1/4 \\
y = -1, &x^\top e_1 = +1, &x^\top e_2 = -1 & \textup{ w/ prob. } 1/4 \\
y = -1, &x^\top e_1 = -1, &x^\top e_2 = +1 & \textup{ w/ prob. } 1/4 \\
\end{array}
\end{align*}

Figure \ref{fig:cDvis} shows samples from $\cD$ when there are 3 dimensions. From the visualization, it is clear that there is no linear separator for $\cD$. As Lemma~\ref{lem:l1smallnorm} shows, a~\relu~network with four neurons can fit this relatively complicated decision boundary. On the other hand, for kernel methods, we prove that the symmetries in $\cD$ induce cancellation in feature space. As a result, the features are less predictive of the true label and the margin will therefore be small. We formalize this argument in Section~\ref{subsec:class-compare-proofs}. 

\paragraph{Gap in regression setting:}
We are able to prove an even larger $\Omega(\sqrt{n/d})$ gap between neural networks and kernel methods in the regression setting where we wish to interpolate continuous labels. Analogously to the classification setting, optimizing a regularized squared error loss on neural networks is equivalent to solving a minimum 1-norm regression problem (see Theorem~\ref{thm:nnl1normregression}). Furthermore, kernel methods correspond to a minimum 2-norm problem. We construct distributions $\pdata$ where the 1-norm solution will have a generalization error bound of $O(\sqrt{d/n})$, whereas the 2-norm solution will have a generalization error bound that is $\Omega(1)$ and thus vacuous. In Section~\ref{subsec:reg-compare-proofs}, we define the 1-norm and 2-norm regression problems. In Theorem~\ref{thm:formalreggap} we formalize our construction.






==> generalization_deep.tex <==
\section{Generalization Properties of a Maximum Margin Neural Network}
\label{sec:generalizationdeep}

\Tnote{I wonder whether we need this section to stand alone. I think we can Prop 3.1 can go to appendix, and Corollary 3.2 can be a corollary of Theorem 2.1? }

\Tnote{we could move the  Proposition 3.1 to a  preliminary section}

\Tnote{I think 3.2 can be merged into previous section. 3.3 can still be in a single section but then the section can be very short, which is probably okay.}

In Section~\ref{sec:margin} we showed that optimizing a weakly-regularized logistic loss leads to the maximum normalized margin. We now study the direct implications of this result on the generalization of the solution. Specifically, we use existing Rademacher complexity bounds of \citet{golowich2017size} to present a generalization bound that depends on the network architecture only through the inverse $\ell_2$-normalized margin and depth of the network (see Proposition~\ref{prop:genbound}). Next, we combine this bound with Theorem~\ref{thm:multilabelmargin} to conclude that parameters obtained by optimizing logistic loss with weak $\ell_2$-regularization will have a generalization bound that scales with the inverse of the maximum possible margin and depth. Finally, we note that the maximum possible margin can only increase with the size of the network, which suggests that increasing the size of the network improves generalization of the solution (see Theorem~\ref{thm:marginnondecreasing}). 






By applying Theorem~\ref{thm:opterrrequired} with Proposition~\ref{prop:genbound}, we can also conclude that optimizing $L_{\lambda, \mathcal{M}}$ within a constant factor gives a margin, and therefore generalization bound, approximating the best possible. 

One consequence of Corollary~\ref{cor:margingeneralization} is that optimizing weakly-regularized logistic loss results in the best possible generalization bound out of all models with the given architecture. This indicates that the widely used algorithm of optimizing deep networks with $\ell_2$-regularized logistic loss has an implicit bias towards solutions with good generalization. 

Next, we observe that the maximum normalized margin is non-decreasing with the size of the architecture. Formally, for two depth-$K$ architectures $\mathcal{M} = (m_1, \ldots, m_{K - 1})$ and $\mathcal{M'} = (m'_1, \ldots, m'_{K - 1})$, we say $\mathcal{M} \le \mathcal{M'}$ if $m_i \le m'_i \ \forall i = 1, \ldots K-1$. Theorem~\ref{thm:marginnondecreasing} states that if $\mathcal{M} \le \mathcal{M'}$, then the max-margin over networks with architecture $\mathcal{M'}$ is at least the max-margin over networks with architecture $\mathcal{M}$. 

\begin{theorem}
	\label{thm:marginnondecreasing}
	Recall that $\gamma^{\star,\mathcal{M}}$ denotes the maximum normalized margin of a network with architecture $\mathcal{M}$.
	If $\mathcal{M} \le \mathcal{M'}$, we have
$
		\gamma^{\star,\mathcal{M}} \le \gamma^{\star,\mathcal{M'}}
.$
	As a important consequence, the generalization error bound of Corollary~\ref{cor:margingeneralization} for $\mathcal{M'}$ is at least as good as that for $\mathcal{M}$.
\end{theorem}
This theorem is simple to prove and follows because we can directly implement any network of architecture $\mathcal{M}$ using one of architecture $\mathcal{M'}$, if $\mathcal{M}\le \mathcal{M'}$. This can explain why additional over-parameterization has been empirically observed to improve generalization in two-layer networks \citep{neyshabur2017exploring}: the margin does not decrease with a larger network size, and therefore Corollary~\ref{cor:margingeneralization} gives a better generalization bound. In Section~\ref{sec:experiments}, we provide empirical evidence that the test error decreases with larger network size while the margin is non-decreasing.

The phenomenon in Theorem~\ref{thm:marginnondecreasing} contrasts with standard $\ell_2$-normalized linear prediction. In this setting, adding more features increases the norm of the data, and therefore the generalization error bounds could also increase. On the other hand, Theorem~\ref{thm:marginnondecreasing} shows that adding more neurons (which can be viewed as learned features) can only improve the generalization of the max-margin solution.




==> proofcomparison.tex <==
\section{Missing Proofs for Comparison to Kernel Methods}
\subsection{Classification}
\label{subsec:class-compare-proofs}
In this section we will complete a proof of Theorem~\ref{thm:l1-l2}. Recall the construction of the distribution $\cD$ provided in Section~\ref{subsec:classificationcompare}. We first provide a classifier of this data with small $\ell_1$ norm.


Now we will upper bound the margin attainable by the $\ell_2$ SVM.
\begin{lemma}[Margin upper bound tool]\label{lem:1}
	In the setting of Theorem~\ref{thm:l1-l2},  we have
	\begin{align*}
	\opt_{\ell_2} \le \frac{1}{\sqrt{\kappa}} \cdot \left\|\frac{1}{n}\sum_{i=1}^n \varphi(x_i)y_i\right\|_2
	\end{align*}
\end{lemma}
\begin{proof}
	By the definition of $\gamma_{\ell_2}$, we have that for any $\alpha$ with $\sqrt{\kappa}\|\alpha\|_2\le 1$, we have
	\begin{align*}
	\gamma_{\ell_2} \le \max_{\sqrt{\kappa}\|\alpha\|_2 \le 1} \frac{1}{n}\sum_{i=1}^{n} \langle \alpha, y_i \varphi(x_i)\rangle
	\end{align*}
	Setting  $\alpha = \frac{1}{\sqrt{\kappa}}\frac{1}{n}\sum_{i=1}^n \varphi(x_i)y_i/ \|\frac{1}{n}\sum_{i=1}^n \varphi(x_i)y_i\|_2$ completes the proof. (Attentive readers may realize that this is equivalent to setting the dual variable of the convex program~\ref{eq:kernel} to all 1's function.)
\end{proof}

\begin{lemma}\label{lem:cancellation}
	In the setting of Theorem~\ref{thm:l1-l2}, 	let $(x_i,y_i)_{i= 1}^n$ be $n$ i.i.d samples and corresponding labels from $\cD$. 	Let $\varphi$ be defined in~\eqref{eqn:def:varphi} with $\phi = \relu$. With high probability (at least $1-dn^{-10}$), we have 
	\begin{align*}
	\left\|\frac{1}{n}\sum_{i=1}^n \varphi(x_i)y_i\right\|_2  \lesssim \sqrt{\kappa/n}\log n +\sqrt{\kappa}/d
	\end{align*}
\end{lemma}
\begin{proof}
	Let $W_i = \varphi(x_i)y_i$. We will bound several quantities regarding $W_i$'s. In the rest of the proof, we will condition on the event $E$ that $\forall i, \|x_i\|_2^2\lesssim d\log n$. Note that $E$ is a high probability event and conditioned on $E$, $x_i$'s are still independent. We omit the condition on $E$ in the rest of the proof for simplicity. 
	
	We first show that assuming the following three inequalities that the conclusion of the Lemma follows.
	\begin{itemize}
		\item[1.] $\forall i, \|W_i\|_2^2\lesssim \kappa\log n$ . 
		\item[2.] $\sigma^2 \triangleq \Var[\sum_i W_i ]\triangleq \sum_{i=1}^n  \Exp [\|W_i - \Exp W_i\|_2^2]\lesssim n\kappa\log n$
		\item[3.] $\|\Exp\left[\sum W_i \right]\|_2 \lesssim \sqrt{\kappa}n/d$. 
	\end{itemize}
	By bullets 1, 2, and Bernstein inequality, we have that with probability at least $1-dn^{-10}$ over the randomness of the data $(X,Y)$, 
	\begin{align*}
	\left\|\sum_{i=1}^n W_i - \Exp\left[\sum_{i=1}^n W_i\right]\right\|_2\lesssim \sqrt{\kappa}\log^{1.5} n + \sqrt{n\kappa\log^2 n} \lesssim \sqrt{n\kappa\log^2 n} 
	\end{align*}
	By bullet 3 and equation above, we complete the proof with triangle inequality:
	\begin{align*}
	\left\|\sum_{i=1}^n W_i\right\|_2 \le  \left\|\Exp\left[\sum_{i=1}^n W_i\right]\right\|_2 + \sqrt{n\kappa\log^2 n} \lesssim \sqrt{n\kappa\log^2 n} +\sqrt{\kappa}n/d
	\end{align*}
	Therefore, it suffices to prove bullets 1, 2 and 3. Note that 2 is a direct corollary of 1 so we will only prove 1 and 3. We start with 3: 
	
	By the definition of the $\ell_2$ norm in $\spacetwo(\sph)$ and the independence of $(x_i,y_i)$'s, we can rewrite 
	\begin{align}
	\left\|\Exp\left[\sum_{i=1}^n W_i\right]\right\|_2^2& = \kappa \cdot n^2 \Exp_{\bdir\sim \sph}\left[\Exp_{(x,y)\sim \cD} \varphi(x)[\bdir]\cdot y\right]^2 \label{eq:4}
	\end{align}
	
	\newcommand{\wtwo}{\bdir_{-2}}
	\newcommand{\xtwo}{x_{-2}}
	
	Let $\bdir = (\bdir_1,\dots, \bdir_d)$ and  $\wtwo = (\bdir_3, \dots, \bdir_d) \in \R^{d-2}$, and define $\tau \triangleq \|\wtwo\|_2$. Let $\xtwo = (x^\top e_3, \dots, x^\top e_d)$. Note that $\varphi(x)[\bdir] y = y [\bdir_1\cdot x^\top e_1 + \bdir_2 \cdot x^\top e_2 + \wtwo^\top \xtwo]$ and $\wtwo^\top \xtwo$ has distribution $\|\wtwo\|_2 \cdot \cN(0,1) = \tau \cdot \cN(0,1)$. Let $z = \wtwo^\top \xtwo/\tau$, and therefore $z$ has standard normal distribution.   With this change of the variables, by the definition of the distribution $\cD$, we have
	
	\begin{align*}
	\begin{split}
	\Exp_{(x,y)\sim \cD} \varphi(x)[\bdir]\cdot y& = \frac{1}{4}\Exp_{z\sim N(0,1)}[(\bdir_1+\bdir_2+\tau z)_+] + \frac{1}{4}\Exp_{z\sim N(0,1)}[(-\bdir_1-\bdir_2+\tau z)_+] \\
	& - \frac{1}{4}\Exp_{z\sim N(0,1)}[(\bdir_1-\bdir_2+\tau z)_+] - \frac{1}{4}\Exp_{z\sim N(0,1)}[(+\bdir_1-\bdir_2+\tau z)_+] 	\end{split} \end{align*}
	By claim~\ref{claim:cancelation}, and the 1-homogeneity of \relu, we can simplify the above equation to 
	\begin{align}
	\Exp_{(x,y)\sim \cD} \varphi(x)[\bdir]\cdot y & = \frac{1}{4}\tau \cdot \left(2c_1 + O(\min \{|\bdir_1+\bdir_2|/\tau, |\bdir_1+\bdir_2|^2/\tau^2\}) \right.\nonumber\\
	& \left. -\frac{\tau}{4}\left( 2c_1 - O(\min \{|\bdir_1-\bdir_2|/\tau, |\bdir_1-\bdir_2|^2/\tau^2\})\right) \right)\nonumber\\
	&\lesssim \min\{|\bdir_1|+|\bdir_2|, (|\bdir_1|+|\bdir_2|)^2/\tau\}\nonumber
	\end{align}
	It follows that 
	\begin{align}
	& \Exp_{\bdir\sim \sph}\left[\Exp_{(x,y)\sim \cD} \varphi(x)[\bdir]\cdot y\right]^2   \lesssim \E_{\bdir} \left[\min\{(|\bdir_1|+|\bdir_2|)^2, (|\bdir_1|+|\bdir_2|)^4/\|\wtwo\|_2^2\}\right] \nonumber\\
	& \lesssim  \E_{\bdir}\left[(|\bdir_1|+|\bdir_2|)^2\cdot \ind{\|\wtwo\|_2\le 1/2}\right] +   \E_{\bdir}\left[(|\bdir_1|+|\bdir_2|)^4/\|\wtwo\|_2^2 \cdot \ind{\|\wtwo\|_2 \ge 1/2}\right] \nonumber\\
	& \lesssim  \exp(-\sqrt{d})+ \E_{\bdir}\left[(|\bdir_1|+|\bdir_2|)^4\right] \lesssim 1/d^2 \label{eq:2}
	\end{align}
	Combining~\eqref{eq:4} and~\eqref{eq:2} we complete the proof of bullet 3. 
	Next we prove bullet 1. 
	Note that $\varphi(x)[\bdir]y$ is bounded by $|\bdir_1|+|\bdir_2| + \|\wtwo^\top \xtwo\|_2$. Therefore, conditioned on $\|x_i\|_2\lesssim d\log n$
	\begin{align}
	\|W_i\|_2^2 & \le \Exp_{\bdir\sim \sph} \left[(|\bdir_1|+|\bdir_2| + \|\wtwo^\top \xtwo\|_2)^2\right] \nonumber\\
	& \lesssim \Exp_{\bdir\sim \sph} \left[|\bdir_1|^2\right]+ \Exp_{\bdir\sim \sph} \left[|\bdir_2|^2\right] + \Exp_{\bdir\sim \sph} \left[\|\wtwo^\top \xtwo\|_2^2\right] \nonumber\\
	& \lesssim 1/d + \|\xtwo\|_2^2/d \lesssim \log n\nonumber
	\end{align}
	Hence we complete the proof.
\end{proof}



\begin{claim}\label{claim:cancelation}
	Let $Z\sim \cN(0,1)$ and $a\in \R$. Then, there exists a universal constant $c_1$ and $c_2$ such that 
	\begin{align*}
	|\E\left[(a+Z)_+ + (-a+Z)_+\right] - 2c_1| \le c_2 \min\{|a|, a^2\}. 
	\end{align*}
\end{claim}

\begin{proof}
	Without loss of generality we can assume $a \ge 0$. Then, 
	\begin{align*}
	& \E\left[(a+Z)_+ + (-a+Z)_+\right]  = \E\left[(a+Z) \ind{Z\ge -a}\right] +  \E\left[(Z-a) \ind{Z\ge a}\right] \nonumber\\
	& = \E\left[a\cdot \ind{Z\ge -a}\right] + \Exp\left[Z \cdot \ind{Z\ge -a}\right] - \E\left[a\cdot \ind{Z\ge a}\right] + \Exp\left[Z\cdot \ind{Z\ge a}\right] \nonumber\\
	& = \E\left[a \ind{-a \le Z\le a}\right] + 2\Exp\left[Z\cdot \ind{Z\ge a}\right] \tag{by $\Exp\left[Z\cdot \ind{-a\le Z\le a}\right]=0$}\\
	& = \E\left[a \ind{-a \le Z\le a}\right] + 2\Exp\left[Z\cdot \ind{Z\ge 0}\right] - 2\Exp\left[Z\cdot \ind{a \ge Z\ge 0}\right] \\
	& = 2c_1 + O(\min\{a, a^2\})
	\end{align*}
	where the last equality uses the fact that $c_1 \triangleq \Exp\left[Z\cdot \ind{Z\ge 0}\right]$ and $\E\left[a \ind{-a \le Z\le a}\right] \le a \E\left[\ind{-a \le Z\le a}\right] \lesssim a \min\{1, a\}$.
\end{proof}

Now we will prove Theorem \ref{thm:l1-l2}. 
\begin{proof}[Proof of Theorem \ref{thm:l1-l2}]
	
	 We can therefore apply Proposition~\ref{prop:genbound}, and conclude that with probability $1 - \delta$, 
	\begin{align*}
		L_{\ell_1\textup{-svm}} \lesssim \sqrt{\frac{d\log n}{n}} + \sqrt{\frac{\log \log (d \log n)}{n}} + \sqrt{\frac{\log (1/\delta)}{n}}
	\end{align*}
	Furthermore, plugging $\gamma_{\ell_2}$ into the bound of Lemma~\ref{lem:generror-l2-svm} gives us 
	\begin{align*}
		\min\left \{1, d \sqrt{\frac{\log n}{n}} \right\} +  \sqrt{\frac{\log \log (dn)}{n}} + \sqrt{\frac{\log (1/\delta)}{n}}
	\end{align*}
\end{proof}

\subsection{Regression}
\label{subsec:reg-compare-proofs}
We will first define the 1-norm and 2-norm regression problems. 
The regression equivalent of \eqref{eq:l1svm} for $\alpha \in \spaceone(\sph)$ is as follows:
\begin{align}
\begin{split}
\alpha_{\ell_1} \in & \argmin_{\alpha} \|\alpha\|_1 \\ 
&\subj \langle \alpha, \varphi(x_i) \rangle = y_i 
\label{eq:l1reg}
\end{split}
\end{align}
Next we define the regression version of \eqref{eq:kernel}:
\begin{align}
\begin{split}
\alpha_{\ell_2} \in& \argmin_{\alpha} \|\alpha\|_2 \\ 
&\subj \langle \alpha, \varphi(x_i) \rangle = y_i 
\label{eq:kernelreg}
\end{split}
\end{align}
where $\alpha \in \spacetwo(\sph)$.

We will briefly motivate our study of the regression setting by connecting the minimum 1-norm solution to neural networks. To compare, in the classification setting, optimizing the weakly regularized loss over neural networks is equivalent to solving the $\ell_1$ SVM. In the regression setting, solving the weakly regularized squared error loss is equivalent is equivalent to finding the minimum 1-norm solution that fits the datapoints exactly.



We proceed to provide similar generalization bounds as the classification setting. This time, our bounds depend on the norms of the solution rather than the margin.  Let $f^{\phi}(\alpha; \cdot) \triangleq x \mapsto \langle \alpha, \varphi(x) \rangle$ (for $\varphi(x)$ defined in~\eqref{eqn:def:varphi}). Following the convention in Section~\ref{subsec:kernelgenbound}, define hypothesis class $\hyp^{1, \phi}_B \triangleq \{f^{\phi}(\alpha; \cdot) : \alpha \in \spaceone(\sph), \|\alpha\|_1 \le B\}$ of linear functionals bounded by $B$ in $1$-norm. As before, define $\hyp^{2, \phi}_B$ and let $\erad(\hyp)$ denote the empirical Rademacher complexity of hypothesis class $\hyp$. 

We will first derive a Rademacher complexity bound for $\hyp^{1, \phi}_B$. 
\begin{claim}
	\label{claim:l1rad}
	$\erad(\hyp^{1, \phi}_{B}) \le \frac{1}{n} B \E_{\epsilon_i}  \left[\left\|\sum_{i = 1}^n \epsilon_i \varphi(x_i)\right\|_{\infty}\right]$.
\end{claim}
\begin{proof}
	We write
	\begin{align}
	\erad(\hyp^{1, \phi}_B) &= \frac{1}{n}\E_{\epsilon_i} \left[\sup_{\alpha \in \hyp^{1, \phi}_B} \langle \alpha, \sum_{i = 1}^n \epsilon_i \varphi(x_i) \rangle \right]\notag \\
	&\le \frac{1}{n} \E_{\epsilon_i} \left[\sup_{\alpha \in \hyp_B^{1, \phi}} \|\alpha\|_1 \left\|\sum_{i = 1}^n \epsilon_i \varphi(x_i)\right\|_{\infty} \right]\notag \\
	&\le \frac{1}{n} B\cdot \E_{\epsilon_i} \left[\left\|\sum_{i = 1}^n \epsilon_i \varphi(x_i)\right\|_{\infty}\right] \notag
	\end{align}
\end{proof}
We will now complete the bound on $\erad(\mathcal{F}^{1, \phi}_B)$ for Lipschitz activations $\phi$ with $\phi(0) = 0$. 
\begin{claim}
	\label{claim:phil1rad}
	Suppose that our activation $\phi$ is $M$-Lipschitz and $\phi(0) = 0$.Then 
	\begin{align*}
	\erad(\mathcal{F}^{1, \phi}_B) \le \frac{3BM\sqrt{\sum_{i = 1}^n\|x_i\|_2^2}}{n}
	\end{align*} 
\end{claim}
\begin{proof}
	We will show that
	\begin{align*}
	E_{\epsilon_i}\left[\left\|\sum_{i = 1}^n \epsilon_i \varphi(x_i) \right\|_{\infty}\right] \le 3M\sqrt{\sum_{i = 1}^n\|x_i\|_2^2}
	\end{align*}
	from which the statement of the lemma follows via Claim \ref{claim:l1rad}. Fix any $\bdir' \in \sph$. Then we get the decomposition
	\begin{equation}
	\begin{split}
	E_{\epsilon_i} \left[\sup_{\bdir \in \sph} \left| \sum_{i = 1}^n \epsilon_i \phi(\bdir^{\top}x_i) \right|\right] &\le E_{\epsilon_i} \left[\left|\sum_{i = 1}^n \epsilon_i \phi(\bdir'^{\top}x_i) \right|\right] + \\
	&E_{\epsilon_i} \left[\sup_{\bdir \in \sph} \left| \sum_{i = 1}^n \epsilon_i \phi(\bdir^{\top}x_i) \right| - \inf_{\bdir \in \sph} \left| \sum_{i = 1}^n \epsilon_i \phi(\bdir^{\top}x_i) \right|\right] 
	\label{eq:supdecomp}
	\end{split}
	\end{equation}
	We can bound the first term as 
	\begin{align}
	E_{\epsilon_i} \left[\left|\sum_{i = 1}^n \epsilon_i \phi(\bdir'^{\top}x_i)\right|\right] &\le \sqrt{E_{\epsilon_i }\left[\left(\sum_{i = 1}^n \epsilon_i \phi(\bdir'^{\top}x_i)\right)^2\right]} \notag \\
	&\le \sqrt{\sum_{i = 1}^n \phi(\bdir'^{\top}x_i)^2} \notag \\
	&\le M\sqrt{\sum_{i = 1}^n (\bdir'^{\top}x_i)^2} \tag{since $\phi$ is Lipschitz and $\phi(0) = 0$} \\
	&\le M \sqrt{\sum_{i = 1}^n \|x_i\|_2^2} \label{eq:fixthetabound}
	\end{align}
	We note that the second term of \eqref{eq:supdecomp} can be bounded by 
	\begin{align}
	\E_{\epsilon_i}& \left[\sup_{\bdir\in \sph} \left| \sum_{i = 1}^n \epsilon_i \phi(\bdir^{\top}x_i)\right| - \inf_{\bdir \in \sph} \left| \sum_{i = 1}^n \epsilon_i \phi(\bdir^{\top}x_i) \right|\right] \nonumber \\&\le \E_{\epsilon_i} \left[\sup_{\bdir \in \sph} \sum_{i = 1}^n \epsilon_i \phi(\bdir^{\top}x_i) - \inf_{\bdir \in \sph} \sum_{i = 1}^n \epsilon_i \phi(\bdir^{\top}x_i)\right] \nonumber 
	\end{align}
	This follows from the general fact that the difference between the supremum and infimum of the absolute value of a quantity is bounded by the difference between the supremum and the infimum. Furthermore, by symmetry of the Rademacher random variables, 
	\begin{align}
	\E_{\epsilon_i} \left[\sup_{\bdir \in \sph} \sum_{i = 1}^n \epsilon_i \phi(\bdir^{\top}x_i) - \inf_{\bdir \in \sph} \sum_{i = 1}^n \epsilon_i \phi(\bdir^{\top}x_i)\right] &\le 2\E_{\epsilon_i} \left[\sup_{\bdir \in \sph} \sum_{i = 1}^n \epsilon_i \phi(\bdir^{\top}x_i)\right] \label{eq:radsup}
	\end{align}
	This simply gives an empirical Rademacher complexity of the hypothesis class $\hyp \triangleq \{x \mapsto \phi(\bdir^{\top}x) : \bdir \in \sph\}$ scaled by $n$. By the Lipschitz contraction property of Rademacher complexity, using the fact that $\phi$ is $M$-Lipschitz, we can therefore bound \eqref{eq:radsup} by 
	\begin{equation}
	2\E_{\epsilon_i} \left[\sup_{\bdir \in \sph} \sum_{i = 1}^n \epsilon_i \phi(\bdir^{\top}x_i)\right] \le 2M\sqrt{\sum_{i = 1}^n \|x_i\|_2^2}
	\label{eq:supminusinfbound}
	\end{equation}
	Plugging \eqref{eq:fixthetabound} and \eqref{eq:supminusinfbound} back into \eqref{eq:supdecomp} gives the desired bound. 
\end{proof}

The following is a generalization bound based on the 1-norm:
\begin{lemma}
	\label{lem:onenormregbound}
	Let $l(\cdot; y) : \R \rightarrow [-c, c]$ be a bounded $M$-Lipschitz loss function. Assume that $\phi$ is a 1-Lipschitz activation with $\phi(0) = 0$. Let $(x_i, y_i)_{i= 1}^n$ be drawn i.i.d from $\pdata$. Then with probability at least $1 - \delta$ over the dataset, every $\alpha \in \spaceone(\sph)$ satisfies 
	\begin{align*}
	&\E_{(x, y) \sim \pdata} [l(f^{\phi}(\alpha; x); y)] \le \\ 
&	\frac{1}{n} \sum_{i = 1}^n l(f^{\phi}(\alpha; x_i); y_i) + 12M\frac{\max\{1, \|\alpha\|_1 \|X\|_F\}}{n} + c\sqrt{\frac{\log(1/\delta) +\log(\max\{1, 2\|\alpha\|_1 \|X\|_F\}) }{2n}}
	\end{align*}
\end{lemma} 
\begin{proof}
	Our starting point is Theorem 1 of \citet{kakade2009complexity}, which states that with probability $1 - \delta$, for any fixed hypothesis class $\hyp$ and $f \in \hyp$, 
	\begin{align}
	\label{eq:fixedhyprad}
		\E_{(x, y) \sim \pdata} [l(f(x); y)] \le \frac{1}{n} \sum_{i = 1}^n l(f(x_i); y_i) + 2M\erad(\hyp) + c \sqrt{\frac{\log(1/\delta)}{n}}
	\end{align}
	We define $B_j \triangleq \frac{2^j}{\|X\|_F}$ for $j \ge 0$. We note that by Claim~\ref{claim:phil1rad}, $\erad(\hyp^{1, \phi}_{B_j}) \le 3\frac{2^j}{n}$. and apply the above on $\hyp^{1, \phi}_{B_j}$ using $\delta_j \triangleq \frac{\delta}{2^{j + 1}}$. Then using a union bound, with probability $1 - \sum_{j= 0}^{\infty} \delta_j = 1- \delta$, for all $j\ge 0$ and $f^{\phi}(\alpha; \cdot) \in \hyp^{1, \phi}_{B_j}$
	\begin{align*}
	\E_{(x, y) \sim \pdata} [l(f^{\phi}(\alpha; x); y)] &\le \frac{1}{n} \sum_{i = 1}^n l(f^{\phi}(\alpha; x_i); y_i) + 2M\erad(\hyp^{1, \phi}_{B_j}) + c \sqrt{\frac{\log(1/\delta_j)}{n}} \\
	&\le \frac{1}{n} \sum_{i = 1}^n l(f^{\phi}(\alpha; x_i); y_i) + 6M\frac{2^j}{n}  + c \sqrt{\frac{\log(1/\delta) + \log(2^{j+ 1})}{n}}
	\end{align*}
	Now for every $\alpha$ with $\|\alpha\|_1 < \frac{1}{\|X\|_F}$, we use the inequality for $\hyp^{1, \phi}_{B_0}$, and for every other $\alpha$, we apply the inequality corresponding to $\hyp^{1, \phi}_{B_{j + 1}}$, where $2^j \le \|\alpha\|_1 \|X\|_F \le 2^{j+ 1}$. This gives the desired statement.
\end{proof}
We can also provide the same generalization error bound for the 2-norm and~\relu~features: 
\begin{lemma}
	\label{lem:twonormregbound}
	In the setting of Lemma \ref{lem:onenormregbound}, choose $\phi$ to be the~\relu~activation. Then with probability $1 - \delta$, every $\alpha \in \spacetwo(\sph)$ satisfies
	\begin{align*}
	&	\E_{(x, y) \sim \pdata} [l(f^{\phi}(\alpha; x); y)] \lesssim \\& 
		\frac{1}{n} \sum_{i = 1}^n l(f^{\phi}(\alpha; x_i); y_i) + M\frac{\sqrt{\kappa}\max\{1, \|\alpha\|_2 \|X\|_F\}}{n\sqrt{d}} + c\sqrt{\frac{\log(1/\delta) +\log(\max\{1, \|\alpha\|_2 \|X\|_F\}) }{2n}}
	\end{align*}
\end{lemma}
\begin{proof}
	We proceed the same way as in the proof of Lemma \ref{lem:onenormregbound}. We define $B_j$ as before, and this time have $\erad(\hyp^{2, \phi}_{B_j}) \lesssim \frac{\sqrt{\kappa}2^j}{n\sqrt{d}}$ from Corollary \ref{cor:relunormboundsl1}. Thus, again union bounding over all $j$, equation \eqref{eq:fixedhyprad} gives with probability $1 - \delta$, for all $j \ge 0$ and $f^{\phi}(\alpha; \cdot) \in \hyp^{2, \phi}_{B_j}$
	\begin{align*}
		\E_{(x, y) \sim \pdata} [l(f^{\phi}(\alpha; x); y)] &\lesssim \frac{1}{n} \sum_{i = 1}^n l(f^{\phi}(\alpha; x_i); y_i) + M\frac{\sqrt{\kappa} 2^j}{n \sqrt{d}} + c \sqrt{\frac{\log(1/\delta) + \log(2^{j+ 1})}{n}} 
	\end{align*}
	Now we assign the $\alpha$ to different $j$ as before to obtain the statement in the lemma.
\end{proof}

Note that if $l$ is some bounded loss such that $l(y; y)= 0$ (for example, truncated squared error), for $\alpha_{\ell_1}$ and $\alpha_{\ell_2}$ the loss terms over the datapoints (in the bounds of Lemmas~\ref{lem:onenormregbound} and~\ref{lem:twonormregbound}) vanish. For loss $l$, define 
\begin{align*}
	L_{\ell_1\textup{-reg}} \triangleq \E_{x, y \sim \pdata}[l(f^{\phi}(\alpha_{\ell_1}; x); y)] \\
	L_{\ell_2\textup{-reg}}\triangleq \E_{x, y \sim \pdata}[l(f^{\phi}(\alpha_{\ell_2}; x); y)]
\end{align*}
Next, we will define the kernel matrix $K$ with $K_{ij} = \langle \varphi(x_i), \varphi(x_j) \rangle$. Now we are ready to state and prove the formal theorem describing the gap between the 1-norm solution and 2-norm solution. 
\begin{theorem}
	\label{thm:formalreggap}
Recall the definitions of $\alpha_{\ell_1}$ and $\alpha_{\ell_2}$ in \eqref{eq:l1reg} and \eqref{eq:kernelreg}. For any activation $\phi$ with the property that $K$ is full rank for any $X$ with no repeated datapoints, there exists a distribution $\pdata$ such that with probability 1,
\begin{align*}
\|\alpha_{\ell_1}\|_1 \le 1
\end{align*}
On the other hand, 
\begin{align*}
\E_{(x_i, y_i)_{i = 1}^n \sim_{\text{iid}} \pdata}[\|\alpha_{\ell_2}\|_2^2] = \frac{n}{\kappa}
\end{align*} 
For i.i.d samples from this choice of $\pdata$, if $l$ is bounded ($l(\cdot ;y) : \R\rightarrow [-1, 1]$), 0 on correct predictions ($l(y; y) = 0$), and 1-Lipschitz, then with probability $1- \delta$, 
\begin{align*}
	L_{\ell_1\textup{-reg}} \lesssim \sqrt{\frac{d}{n}} + \sqrt{\frac{\log(1/\delta) + \log n}{n}}
\end{align*}
Meanwhile, in the case that $\|\alpha_{\ell_2}\|_2^2 \ge \frac{n}{\kappa}$, the upper bound on $L_{\ell_2\textup{-reg}}$ from Lemma \ref{lem:twonormregbound} is $\Omega(1)$ and in particular does not decrease with $n$.
\end{theorem}

We will first show that for any dataset $X$, there is a distribution over $Y$ such that the expectation of $\|\alpha_{\ell_2}\|_2$ is large. When it is clear from context, $y$ will denote the vector corresponding to $Y$.

\newcommand{\cA}{\mathcal{A}}
\begin{lemma}
	\label{lem:l1l2gap}
	There is a distribution $\mathcal{A}$ over $\spaceone(\sph)$ such that for any dataset $X$ with $y_i \triangleq \langle\varphi(x_i), \beta \rangle$ for $\beta \sim \cA$, 
	\begin{align*}
		\E_{\beta}[\|\alpha_{\ell_2}\|^2_2] \ge \frac{n}{\kappa}
	\end{align*} 
	and with probability 1,
	\begin{align*}
		\|\alpha_{\ell_1}\|_1 \le 1
	\end{align*}
\end{lemma}

We note the order of the quantifiers in Lemma \ref{lem:l1l2gap}: the distribution $\cA$ must not depend on the dataset $X$. We first provide a simple closed-form expression for $\|\alpha_{\ell_2}\|_2^2$. 

\begin{claim}
	\label{claim:alphaell2closedfform}
	If $K$ is full rank, then $\|\alpha_{\ell_2}\|_2^2 = y^{\top} K^{-1} y$. 
\end{claim}
\begin{proof}
	This follows by taking the dual of \eqref{eq:kernelreg}.
\end{proof}

\begin{proof} [Proof of Lemma \ref{lem:l1l2gap}]
	We sample $\beta \sim \cA$ as follows: first sample $\bdir \sim \sph$ uniformly. Then set $\beta$ to have a delta mass of 1 at $\bdir$ and be 0 everywhere else. Define the vector $v_{\bdir} \triangleq [\phi(\bdir^{\top}x_1) \cdots \phi(\bdir^{\top}x_n)]$; then it follows that we set our labels $y$ to $v_{\bdir}$. It is immediately clear that $\|\alpha_{\ell_1}\|_1 \le \|\beta\|_1 \le 1$.
	
	To lower bound $\E_{\beta} [\|\alpha_{\ell_2}\|^2_2]$, from Claim \ref{claim:alphaell2closedfform} we get
	\begin{align*}
		\E_{\beta \sim \cA}[\|\alpha_{\ell_2}\|_2^2] &= E_{\bdir \sim \sph}[v_{\bdir}^{\top} K^{-1} v_{\bdir}] \\
		&= E_{\bdir \sim \sph}[\tr K^{-1}(v_{\bdir}v_{\bdir}^{\top})] \\
		&= \tr(K^{-1} E_{\bdir \sim \sph}[v_{\bdir}v_{\bdir}^{\top}] \\
		&= \frac{1}{\kappa} \tr(K^{-1} K) \tag{by definition of $K$}\\
		&= \frac{n}{\kappa}
	\end{align*}
\end{proof}

\begin{proof}[Proof of Theorem \ref{thm:formalreggap}]
	We note that since the distribution $\cA$ of Lemma \ref{lem:l1l2gap} does not depend on the dataset $X$, it must follow that 
	\begin{align*}
		\E_{(x_i)_{i = 1}^n \sim_{\text{iid}} \mathcal{N}(0, I_{d \times d})} \left[\E_{\beta \sim \cA} [\|\alpha_{\ell_2}\|_2^2]\right] &= \frac{n}{\kappa}\\
		\E_{\beta \sim \cA} \left[\E_{(x_i)_{i = 1}^n \sim_{\text{iid}} \mathcal{N}(0, I_{d \times d})} [\|\alpha_{\ell_2}\|_2^2]\right]&= \frac{n}{\kappa}
	\end{align*} 
	Thus, there exists $\beta^{\star}$ such that if we sample $X$ i.i.d. from the standard normal and set $y_i = \langle \varphi(x_i), \beta^{\star} \rangle$, the expectation of $\|\alpha_{\ell_2}\|_2^2$ is at least $\frac{n}{\kappa}$. We choose $\pdata$ corresponding to this $\beta^{\star}$, with $x$ sampled from the standard normal. Now it is clear that $\pdata$ will satisfy the norm conditions of Theorem \ref{thm:formalreggap}. 
	
	For the generalization bounds, with high probability $\|X\|_F = \Theta(\sqrt{nd})$ as $x$ is sampled from the standard normal distribution. Thus, Lemma \ref{lem:onenormregbound} immediately gives the desired generalization error bounds for $L_{\ell_1\textup{-reg}}$. On the other hand, if $\|\alpha_{\ell_2}\|_2 \ge \sqrt{\frac{n}{\kappa}}$, then the bound of Lemma \ref{lem:twonormregbound} is at least 
	\begin{align*}
		\frac{\sqrt{\kappa} \|\alpha_{\ell_2}\|_2 \|X\|_F}{n \sqrt{d}} \ge \Omega(1)
	\end{align*}
\end{proof}



==> proofl1svm.tex <==
\section{Missing Proof of Proposition~\ref{prop:gammastar=gammal1}}

\label{sec:proofl1svm}
Proposition~\ref{prop:gammastar=gammal1} follows simply from applying Corollary 1 of~\citet{neyshabur2014search} to a hard-margin SVM problem. For completeness, we provide another proof here. 
The proof of Proposition~\ref{prop:gammastar=gammal1} will consist of two steps: first, show that \eqref{eq:l1svm} has an optimal solution with sparsity $n$, and second, show that sparse solutions to \eqref{eq:l1svm} can be mapped to a neural network with the same margin, and vice versa. The following lemma and proof are based on Lemma 14 of \citet{tibshirani2013lasso}.

\begin{lemma}
	\label{lem:n-sparsity}
	Let $\supp(\alpha) \triangleq \{\bdir : |\alpha(\bdir)| > 0\}$. If an optimal solution to \eqref{eq:l1svm} exists, then there exists an optimal solution $\alpha^\star$ with $|\supp(\alpha^\star)| \le n$. 
\end{lemma}

For the proof of this lemma, we find it convenient to work with a minimum norm formulation which we show is equivalent to \eqref{eq:l1svm}: 
\begin{align}
\begin{split}
\min_{\alpha} &\ \|\alpha\|_1\\
\subj & y_i \langle \alpha, \varphi(x_i)\rangle \ge 1 \ \forall i
\label{prob:minnormalpha}
\end{split}
\end{align}
\begin{claim}
	\label{claim:maxminequalsminnormalpha}
	Let $S \subset \spaceone(\sph)$ be the set of optimizers for $\eqref{eq:l1svm}$, and let $S' \subset \spaceone(\sph)$ be the set of optimizers for \eqref{prob:minnormalpha}. If \eqref{prob:minnormalpha} is feasible, for any $\alpha \in S$, $\frac{\alpha}{\gamma_{\ell_1}} \in S'$, and for any $\alpha' \in S'$, $\frac{\alpha'}{\|\alpha'\|_1} \in S$.
\end{claim}

\begin{proof}
	\newcommand{\opttext}{\mathrm{opt}'}
	Let $\opttext$ denote the optimal objective for \eqref{prob:minnormalpha}. We note that $\frac{\alpha'}{\|\alpha'\|_1}$ is feasible for \eqref{eq:l1svm} with objective $\frac{1}{\opttext}$, and therefore $\gamma_{\ell_1} \ge \frac{1}{\opttext}$. Furthermore, $\frac{1}{2\gamma_{\ell_1}} y_i \int_{\bdir \in \sph} \alpha(\bdir) \phi(\bdir^{\top} x_i) d\bdir \ge 1 \ \forall i$, and so $\frac{\alpha}{\gamma_{\ell_1}}$ is feasible for \eqref{prob:minnormalpha} with objective $\frac{1}{\gamma_{\ell_1}}$. Therefore, $\opttext \le \frac{1}{\gamma_{\ell_1}}$. As a result, it must hold that $\opttext = \frac{1}{\gamma_{\ell_1}}$, which means that $\frac{\alpha'}{\|\alpha'\|_1}$ is optimal for \eqref{eq:l1svm}, and $\frac{\alpha}{\gamma_{\ell_1}}$ is optimal for \eqref{prob:minnormalpha}, as desired. 
\end{proof}

First, note that if~\eqref{prob:minnormalpha} is not feasible, then $\gamma_{\ell_1} = 0$ and \eqref{eq:l1svm} has a trivial sparse solution, the all zeros function. Thus, it suffices to show that an optimal solution to \eqref{prob:minnormalpha} exists that is $n$-sparse, since by Lemma \ref{claim:maxminequalsminnormalpha} \eqref{prob:minnormalpha} and \eqref{eq:l1svm} have equivalent solutions up to a scaling. We begin by taking the dual of \eqref{prob:minnormalpha}. 

\begin{claim}
	\label{claim:dualKKT}
	The dual of \eqref{prob:minnormalpha} has form 
	\begin{align*}
	\begin{split}
	\max_{\lambda \in \R^n} & \ \lambda^{\top} \ones \\
	\subj & \left |\sum_{i = 1}^n \lambda_i y_i \phi(\bdir^{\top}x_i)\right| \le 1 \ \forall \bdir \in \sph \\
	& \lambda_i \ge 0
		\end{split}
	\end{align*}
	For any primal optimal solution $\alpha^\star$ and dual optimal solution $\lambda^\star$, it must hold that 
	\begin{align}
	\label{eq:KKT}
	\sum_{i = 1}^n \lambda^{\star}_i y_i \phi(\bdir^{\top}x_i) = \sign(\alpha^\star(\bdir)) \iff \alpha^\star(\bdir) \ne 0
	\end{align}
\end{claim}
\begin{proof}
	The dual form can be solved for by computation. By strong duality, \eqref{eq:KKT} must follow from the KKT conditions.  
\end{proof}

Now define the mapping $v : \sph \rightarrow \R^n$ with $v_i(\bdir) \triangleq y_i \phi(\bdir^{\top} x_i)$. We will show a general result about linearly dependent $v(\bdir)$ for $\bdir \in \supp(\alpha^\star)$, after which we can reduce directly to the proof of \citet{tibshirani2013lasso}. 
\begin{claim}
	\label{claim:coefficientsum}
	Let $\alpha^\star$ be any optimal solution. Suppose that there exists $S \subseteq \supp(\alpha^{\star})$ such that $\{v(\bdir) : \bdir \in S\}$ forms a linearly dependent set, i.e.
	\begin{align}
	\label{eq:lindepend}
	\sum_{\bdir \in S} c_{\bdir} v(\bdir) = \zeros
	\end{align}
	for coefficients $c$. Then $\sum_{\bdir \in S} c_{\bdir}\sign(\alpha^{\star}(\bdir))= 0$.
\end{claim}


\begin{proof}
	Let $\lambda^\star$ be any dual optimal solution, then ${\lambda^\star}^{\top} v(\bdir) = \sign(\alpha^{\star}(\bdir)) \ \forall \bdir \in \supp(\alpha^{\star})$ by Claim \ref{claim:dualKKT}. Thus, we apply ${\lambda^\star}^{\top}$ to both sides of \eqref{eq:lindepend} to get the desired statement.
\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:n-sparsity}]
	The rest of the proof follows Lemma 14 in \citet{tibshirani2013lasso}. The lemma argues that if the conclusion of Claim \ref{claim:coefficientsum} holds and an optimal solution $\alpha^{\star}$ has $S \subseteq \supp(\alpha^{\star})$ with $\{v(\bdir) : \bdir \in S\}$ linearly dependent, we can construct a new $\alpha'$ with $\|\alpha'\|_1 = \|\alpha^{\star}\|_1$ and $\supp(\alpha') \subset \supp(\alpha^{\star})$ (where the inclusion is strict). First, we can apply Theorem 2 of \citet{rosset2007l1} to conclude that an optimal $\alpha^{\star}$ exists with finite support (indeed, with support size less than $n + 1$). Thus, if we consider an optimal $\alpha^\star$ with minimal support, it must follow that $\{v(\bdir) : \bdir \in \supp(\alpha^\star)\}$ is a linearly independent set, and therefore $|\supp(\alpha^\star)| \le n$.
\end{proof}

We can now complete the proof of Proposition~\ref{prop:gammastar=gammal1}. 

\begin{proof} [Proof of Proposition~\ref{prop:gammastar=gammal1}.]
	For ease of notation, we will parametrize a two-layer network with $m$ units by top layer weights $w_1, \ldots, w_m \in \R$ and bottom layer weights $u_1, \ldots, u_m \in \R^d$. As before, we use $\genparam$ to refer to the collection of parameters, so the network computes the real-valued function
	\begin{align*}
		f(\genparam; x) = \sum_{j = 1}^m w_j \phi(u_j^\top x)
	\end{align*}
	Note that we simply renamed the variables from the parametrization of~\eqref{eq:nneq}.
	
	We first apply Lemma \ref{lem:n-sparsity} to conclude that \eqref{eq:l1svm} admits a $n$-sparse optimal solution $\alpha^\star$. 
	Because of sparsity, we can now abuse notation and treat $\alpha^\star$ as a real-valued function such that $\sum_{\bdir \in \supp(\alpha^\star)} |\alpha^\star(\bdir)| \le 1$. We construct $\genparam$ corresponding to a two-layer network with $m \ge n$ hidden units and normalized margin at least $\frac{\gamma_{\ell_1}}{2}$. For clarity, we let $W$ correspond to the top layer weights and $U$ correspond to the bottom layer weights. For every $\bdir \in \supp(\alpha)$, we let $\genparam$ have a corresponding hidden unit $j$ with $(w_j, u_j) = \left(\sign(\alpha^\star(\bdir))\sqrt{\frac{|\alpha^\star(\bdir)|}{2}}, \sqrt{\frac{|\alpha^\star(\bdir)|}{2}}\bdir\right)$, and set the remaining hidden units to $\zeros$. This is possible because $m \ge n$. Now 
	\begin{align*}
	f(\genparam; x) = \sum_{j = 1}^m \weight_j \phi(\dir_j^{\top} x) = \frac{1}{2}\sum_{\bdir \in \supp(\alpha^\star)} \alpha^\star(\bdir)\phi(\bdir^{\top}x)
	\end{align*} 
	Furthermore, 
	\begin{align*}
	\|\genparam\|_2^2 = \sum_{j = 1}^m w_j^2 + \|u_j\|_2^2 = \sum_{\bdir \in \supp(\alpha)} \frac{|\alpha^\star(\bdir)|}{2} + \frac{|\alpha^\star(\bdir)|}{2} \|\bdir\|_2^2 = \sum_{\bdir \in \supp(\alpha)} |\alpha^\star(\bdir)| \le 1
	\end{align*}
	Thus it follows that $\genparam$ has normalized margin at least $\gamma_{\ell_1}/2$, so $\gamma^{\star, m} \ge \gamma_{\ell_1}/2$. 
	
	To conclude, we show that $\gamma^{\star, m} \le \gamma_{\ell_1}/2$. Let $\genparam^{\star, m}$ denote the parameters obtaining optimal $m$-unit margin $\gamma^{\star, m}$ with hidden units $(\weight^{\star, m}_j, \dir^{\star, m}_j)$ for $j \in [m]$. We can construct $\alpha$ to put a scaled delta mass of $2\weight^{\star, m}_j \|\dir^{\star, m}_j\|_2$ on $\bdir^{\star, m}_j$ for $j  \in [m]$. It follows that 
	\begin{align*}
	\|\alpha\|_1 = \sum_{j = 1}^m 2|\weight^{\star, m}_j|\|\dir^{\star, m}_j\|_2 \le \sum_{j = 1}^m {\weight^{\star, m}_j}^2 + \|\dir^{\star, m}_j\|_2^2 = \|\genparam^{\star, m}\|_2^2 \le 1
	\end{align*}
	Furthermore, 
	\begin{align*}
	\int_{\sph} \alpha(\bdir) \phi(\bdir^{\top}x) &=  2\sum_{j = 1}^m \weight^{\star, m}_j \|\dir^{\star, m}_j\|_2 \phi((\bdir^{\star, m}_j)^{\top}x) \\&= 2\sum_{j = 1}^m \weight^{\star, m}_j \phi({\dir^{\star, m}_j}^{\top}x) = 2f(\genparam^{\star, m}; x)
	\end{align*} 
	Thus, $\alpha$ is a feasible solution to \eqref{eq:l1svm} with objective value at least $2\gamma^{\star, m}$. Therefore, $\gamma_{\ell_1} \ge 2\gamma^{\star, m}$, so $\gamma^{\star, m} = \gamma_{\ell_1}/2$.
\end{proof}




==> twolayer.tex <==
\section{Neural Net Max-Margin vs. Kernel Methods}
\label{sec:twolayer}
\newcommand{\opt}{\gamma}

We will continue our study of the max-margin neural network via comparison against kernel methods, a context in which margins have already been extensively studied. We show that two-layer networks can obtain a larger margin, and therefore better generalization guarantees, than kernel methods. Our comparison between the two methods is motivated by an equivalence between the $\ell_2$ max-margin of an infinite-width two-layer network and the $\ell_1$-SVM \citep{zhu20041} over the lifted feature space defined by the activation function applied to all possible hidden units \citep{neyshabur2014search,rosset2007l1,bengio2006convex}. The kernel method corresponds to the $\ell_2$-SVM in this same feature space, and is equivalent to fixing random hidden layer weights and solving an $\ell_2$-SVM over the top layer. In Theorem~\ref{thm:l1-l2}, we construct a distribution for which the generalization upper bounds for the $\ell_1$-SVM on this feature space are smaller than those for the $\ell_2$-SVM by a $\Omega(\sqrt{d})$ factor. Our work provides evidence that optimizing all layers of a network can be beneficial for generalization.

There have been works that compare $\ell_1$ and $\ell_2$-regularized solutions in the context of feature selection and construct a feature space for which a generalization gap exists (e.g., see \citet{ng2004feature}). In contrast, we work in the fixed feature space of~\relu~activations, which makes our construction particularly challenging. 

We will use $m$ to denote the width of the single hidden layer of the network. Following the convention from Section~\ref{sec:generalizationdeep}, we will use $\gamma^{\star,m}$ to denote the maximum possible normalized margin of a two-layer network with hidden layer size $m$ (note the emphasis on the size of the single hidden layer). The depth $K=2$ case of Corollary~\ref{cor:margingeneralization} implies that optimizing  weakly-regularized $\ell_2$ loss over width-$m$ two-layer networks gives parameters whose generalization bounds depend on the hidden layer size only through $1/\gamma^{\star,m}$. Furthermore, from Theorem~\ref{thm:marginnondecreasing} it immediately follows that 
$
	\gamma^{\star,1} \le \gamma^{\star,2} \le \cdots \le \gamma^{\star,\infty}
$.
\\
The work of \citet{neyshabur2014search} links $\gamma^{\star,m}$ to the $\ell_1$ SVM over a lifted space. Formally, we define a lifting function $\varphi: \R^d \rightarrow \spaceinf(\sph)$ mapping data to an infinite feature vector: 
\begin{align}
\varphi(x) \in \spaceinf(\sph) \textup{ satisfies } \varphi(x)[\bar{u}] = \phi(\bdir^{\top}x)\label{eqn:def:varphi}
\end{align} 
where $\phi$ is the activation of Section~\ref{sec:generalizationdeep}. We look at the margin of linear functionals corresponding to $\alpha\in \spaceone(\sph)$ . The 1-norm SVM \citep{zhu20041} over the lifted feature $\varphi(x)$ solves for the maximum margin:
\begin{align}
\begin{split}
\opt_{\ell_1}\triangleq& \max_{\alpha} \min_{i\in [n]} y_i\langle \alpha, \varphi(x_i)\rangle \\
& \subj  \|\alpha\|_1 \le 1
\label{eq:l1svm}
\end{split}
\end{align}
where we rely on the inner product and 1-norm defined in Section \ref{subsec:notation}. This formulation is equivalent to a hard-margin optimization on ``convex neural networks'' \citep{bengio2006convex}. \citet{bach2017breaking} also study optimization and generalization of convex neural networks. Using results from~\citet{rosset2007l1, neyshabur2014search, bengio2006convex}, our Theorem~\ref{thm:multilabelmargin} implies that optimizing weakly-regularized logistic loss over two-layer networks  is equivalent to solving \eqref{eq:l1svm} when the size of the hidden layer is at least $n + 1$, where $n$ is the number of training examples. Proposition~\ref{prop:gammastar=gammal1} restates this with the minor improvement that this equivalence\footnote{The factor of $\frac12$ is due the the relation that every unit-norm parameter $\Theta$ corresponds to an $\alpha$ in the lifted space with $\|\alpha\|=2$.} holds when the size of the hidden layer is $n$.
\begin{proposition}
	\label{prop:gammastar=gammal1}
	Let $\opt_{\ell_1}$ be defined in~\eqref{eq:l1svm}. If margin $\gamma_{\ell_1}$ is attainable by some solution $\alpha \in \spaceone(\sph)$, then
$
	\frac{\opt_{\ell_1}}{2} = \gamma^{\star,n} = \cdots = \gamma^{\star,\infty}
$.
\end{proposition}

For completeness, we show Proposition~\ref{prop:gammastar=gammal1} in Section~\ref{sec:proofl1svm}, relying on work of \citet{tibshirani2013lasso} and \citet{rosset2007l1}. 

\input{comparison}







